CRDT-Based Game State Synchronization in Peer-to-Peer VR

Virtual presence demands ultra-low latency, a factor that centralized architectures, by their nature, cannot minimize. Local peer-to-peer architectures offer a compelling alternative, but also pose unique challenges in terms of network infrastructure. This paper introduces a prototype leveraging Conflict-Free Replicated Data Types (CRDTs) to enable real-time collaboration in a shared virtual environment. Using this prototype, we investigate latency, synchronization, and the challenges of decentralized coordination in dynamic non-Byzantine contexts. We aim to question prevailing assumptions about decentralized architectures and explore the practical potential of P2P in advancing virtual presence. This work challenges the constraints of mediated networks and highlights the potential of decentralized architectures to redefine collaboration and interaction in digital spaces.

==> commands/mathdefs.tex <==
\RequirePackage{latexsym}
\RequirePackage{dsfont}

% macros for domain teory, semantics, etc. 

% math code definitions

%%%%%%%%%%%%%%%%%%%%%%%%\mathcode`:="603A          % : as punctuation
\mathcode`.="613A          % . as punctuation
\mathcode`|="326A          % | as a relation

\let\es=\relax    %  possible space before punctuation in displayed formulas

%% relations

\newcommand\tx[1]{\hbox{ #1 }}
\newcommand{\defeq}{\stackrel{.}{=}}

\let\vect=\overrightarrow
\let\iff=\Leftrightarrow        % this redefines the original
\let\implies=\Rightarrow
\let\implied=\Leftarrow

\let\sqleq=\sqsubseteq
\let\sqle=\sqsubset
\let\sqgeq=\sqsupseteq
\let\sqgt=\sqsupset
\let\pleq=\sqleq          % partial-order leq
\let\ple=\sqle            % partial-order le
\let\pgeq=\sqgeq          % partial-order geq
\let\pgt=\sqgt          % partial-order geq


\def\land{\mathrel{\wedge}}
\def\lor{\mathrel{\vee}}
\let\bigland=\bigwedge
\let\biglor=\bigvee

\def\preleq{\mathrel{%      % pre-order leq
  \raise 2pt\hbox{$\mathop\sqsubset\limits_{\hbox{$\sim$}}$}%
}}

% operators

\let\union=\cup
\let\bigunion=\bigcup
\let\join=\sqcup
\let\bigjoin=\bigsqcup
\let\meet=\sqcap
%\let\bigmeet=\bigsqcap
\newcommand{\down}{\mathord{\downarrow}}
\newcommand\dec[1]{{{\Downarrow}#1}}

\newcommand\setsize[1]{\left| #1 \right|}
\newcommand\domxtn{\mathbin{\stackrel{+}{|}}}
%\newcommand\domsub{\mathbin{\stackrel{-}{|}}}
\newcommand\domainsub{\mathop{\lhd\mkern-14mu-}}

% arrows

\newcommand{\map}{\mathrel{\hookrightarrow}}
\newcommand\goesto[1]{{\mathop{\longrightarrow}\limits^{#1}}}
\newcommand\goes{\longrightarrow}

% function constants

\newcommand\auxfun[1]{\expandafter\newcommand\csname #1\endcsname{%
 \mathop{\hbox{$\mathsf{#1}$}}\nolimits}}
 \newcommand\af[1]{\mathop{\hbox{$\mathsf{#1}$}}\nolimits}
 \newcommand\kw[1]{\mathrel{\hbox{$\mathbf{#1}$}}}

\let\max=\relax
\let\min=\relax
\auxfun{max}
\auxfun{min}
\auxfun{dom}
\auxfun{ran}
\auxfun{fst}
\auxfun{snd}

% sets

\newcommand{\pow}[1]{{\cal P}(#1)}
\newcommand{\mpow}[1]{{\cal M}(#1)}
\newcommand{\unit}{\mathds{1}}
\newcommand{\bool}{\mathds{B}}
\newcommand{\nat}{\mathds{N}}
\newcommand{\integer}{\mathds{Z}}
\newcommand{\ids}{\mathds{I}}
\newcommand{\topo}{\mathds{T}}

\newcommand{\false}{\mathsf{False}}
\newcommand{\true}{\mathsf{True}}

\newcommand{\quotient}[2]{#1 / #2}

%%%%%%%%%%%

\newcommand\letin[2]{\mathop{\hbox{$\mathrm{let}$}} #1 \Leftarrow #2 . }
\newcommand\lift[1]{\lfloor #1 \rfloor}

%%%%%%%%%%%%%%%%%%%%%

\newcommand\iffdef{\mathrel{\Longleftrightarrow}}
\newcommand\nullstring{\epsilon}
\newcommand\pfunc{\hookrightarrow}
\newcommand\func{\rightarrow}

%% by me

